A Comprehensive Analysis of Deep Regression

Deep learning revolutionized data science, and recently its popularity has grown exponentially, as did the amount of papers employing deep networks. Vision tasks, such as human pose estimation, did not escape from this trend. There is a large number of deep models, where small changes in the network architecture, or in the data pre-processing, together with the stochastic nature of the optimization procedures, produce notably different results, making extremely difficult to sift methods that significantly outperform others. This situation motivates the current study, in which we perform a systematic evaluation and statistical analysis of vanilla deep regression, i.e. convolutional neural networks with a linear regression top layer. This is the first comprehensive analysis of deep regression techniques. We perform experiments on four vision problems, and report confidence intervals for the median performance as well as the statistical significance of the results, if any. Surprisingly, the variability due to different data pre-processing procedures generally eclipses the variability due to modifications in the network architecture. Our results reinforce the hypothesis according to which, in general, a general-purpose network (e.g. VGG-16 or ResNet-50) adequately tuned can yield results close to the state-of-the-art without having to resort to more complex and ad-hoc regression models.

==> cover_letter_r1.tex <==
\onecolumn

\begin{coverletter}{A Comprehensive Analysis of Deep Regression}{TPAMI-2018-03-0223}
 \begin{answereditor}{Please accompany the revised version with a detailed summary of how you addressed every comment by the reviewers (or explanation why any of the comments should not be addressed, e.g., if you disagree).}
We appreciate the comments and proposals made by the reviewers. We have thoroughly reviewed the document accordingly, which we hope that it substantially improved the initial submission. In general terms, the experimental section was considerably extended. First, a new dataset (MPII) was introduced in the comparison section. Second, other loss functions (L1, Huber) and normalization strategies (layer normalization) were included. Finally, other output representations were considered for the regression task (heat maps). In relation to the writing, we introduced clarifications and corrections throughout the document. We hope that all these modifications satisfy the reviewers. 

Below, we provide precise answers to the questions and issues raised by the reviewers, and we outlined in green all the modifications introduced in the manuscript.
 \end{answereditor}

\begin{answerreviewer}[Author Should Prepare A Major Revision For A Second Review]
\ca{This paper is well-written and easy to read. The following points may summarize it: (i) Focus on Regression using Convolutional Neural Networks, (ii) Systematic evaluation and statistical analysis (Wilcoxon Signed-rank test, confidence intervals), (iii) Three computer vision applications: head pose estimation, facial landmark detection, and full-body 2D human pose estimation. (iv) Two base architectures: VGG-16 and ResNet-50. (v) Considered factors: optimization algorithms (AdaGrad, RMSProp, AdaDelta and Adam); batch size; dropout vs batch normalization; fine-tuning depth; location of regression layer; pooling strategy; and, data pre-processing technique. (vi) Comparison of obtained results against the state-of-the-art on the selected datasets. (vii) Wide discussion of the main findings.}
{We thank the reviewer for this very accurate description of the manuscript, its value and motivation.}

\qa{Just the Mean Square Error (MSE) is used as loss function to train the networks. However, alternative loss functions exist for regression purposes (e.g. L1-smooth). So, in this study, and for completeness, one would expect the evaluation and discussion of other loss functions in addition to MSE.}
{We agree that there are other loss possibilities to train deep architectures for regression. We chose the L2 loss in our initial submission since it is the most commonly used loss in regression problems. However, following the recommendation of the reviewer, we show the results obtained by comparing L1, L2 and Huber losses in Table~\ref{tab:VGG-resnet-loss} and discuss it in~\refcm{results-loss}.}

\qa{Evaluating only pre-trained networks as VGG-16 and ResNet-50 limits the applicability of the study. What would you suggest to the reader if the input data of the target problem had a single channel or any number of channels different to three (e.g. medical images)? Or if for some other reasons would be needed to train a custom regression network from the scratch?}
{ First, with respect to the necessity of training a deep network from scratch, it is important to mention that, when tackling deep regression problems, it is common practice to employ pre-trained networks. Since pre-training is the predominant option, the conclusions of our paper would apply in most cases. Furthermore, it is important to remark that, after analyzing the 979 papers published at CVPR'18, only 12.87\% papers employed deep networks trained from scratch (vs a large majority of cases that employ some sort of fine-tuning over a pre-trained model).  %Since there are 126 papers that include the keywords ``from scratch'', out of 979, we get this 12.87\%. {\color{red}I don't know if we are being rigorous with this figure: we implicitly claim that a paper includes a pre-trained/fine-tuned model only if it's not said the opposite (i.e. if it's not explicitly said that is trained from scratch). Is this way of thinking fair? Maybe, many papers just present a new model whose training from scratch is so obvious that it is not even considered necessary to say it explicitly. What do you think?} Therefore, we humbly consider that the applicability of our study is still very broad.{\color{orange} Well, I am more worried about the fact that, among these papers, we have no idea which ones are doing regression}


Second, we consider that the scenario we present in our submission is the most common one in multiple problems (specially in the computer vision community). This includes the medical image analysis domain, just to continue with the example provided by the reviewer, where the three channel scenario is not negligible: it can be found in the classification of gastrointestinal lesions  (\url{http://www.depeca.uah.es/colonoscopy_dataset/}), the analysis of gene-expression histological images  (\url{http://portal.brain-map.org/}) and the detection of diabetic retinopathy lesions in fundus images (\url{https://idrid.grand-challenge.org/Home/}), just to name a few. In fact, in [1],  the authors concluded that pre-trained  deep  ConvNets,  with  sufficient  fine-tuning, eliminate the need for training from scratch in the medical domain. Their extensive experimental section, employing a three-channel input pre-trained ConvNet, based  on  four  distinct  medical  imaging applications from three different imaging modality systems, demonstrated  that  fine-tuned  ConvNets  are  useful  for medical  image  analysis,  performing  as  well  as  fully  trained ConvNets and even outperforming the latter when limited training data  are  available. In particular, in that paper, when the network was facing a problem whose data were single-channel, the only operation performed was to convert to color each extracted gray-scale patch by concatenating three times the gray channel.

We conclude that fine-tuning standard architectures pre-trained on ImageNet is a very widely used strategy, and we intentionally restrict the scope of this study to this scenario.\\

[1] Tajbakhsh, N., Shin, J. Y., Gurudu, S. R., Hurst, R. T., Kendall, C. B., Gotway, M. B., \& Liang, J. (2016). Convolutional neural networks for medical image analysis: Full training or fine tuning? IEEE Transactions on Medical Imaging, 35(5), 1299-1312.
}

\qa{Sec. 5, wrt Dropout, what exact values have been tested? Just 50\%? Since this is a parameter to be selected, why not exploring additional values? E.g. from 10\% to 90\% in steps of 10.}
{Following the sensible comment of the reviewer, we have extended our experimental set-up to cope with additional dropout values; from 20\% to 80\% in steps of 10. The results are presented in Figure~\ref{fig:dropout-rate} and discussed in~\refcm{dropout-rate}.}

\qa{Sec. 5, wrt Regression Layer, I am not whether it is a mistake or not using alternatively RL or LR.}
{We thank the reviewer for all comments aimed to clarify all aspects of the paper. LR was indeed a typo. While REG  refers to the regression layer (as it did in the previous version), RL (regressed layer) is now replaced by TIR: Target and Input Representation, since we included also the evaluation of heat-maps. See \refcm{tir-desc} and \refcm{results-tir} for the discussion on the various representations and the associated results.}

\qa{Page 7, line 32, maybe I am confused, but did you mean Flatten instead of $FC^2$? As I do not see FC as a pooling strategy.}
{As briefly announced in the previous answer, we have reformulated this part, by also including the heatmap regression experiments suggested by R2. Indeed, we now deal with different target and input representations of the regression layer. As explained in the manuscript, see~\refcm{tir-desc}, we compare the use of heatmaps (as target representations) with different input representations when regressing low-dimensional vectors, namely: global average pooling, global max pooling and the second fully connected layer (in the case of VGG-16).}

\qa{Sec. 5.6, I miss any comment regarding the comparison between the use of Dropout and BatchNorm. What is your suggestion wrt them?}
{We thank the reviewer for pointing out this issue. The main conclusion is that the behavior of BN is very stable for both networks, i.e. regardless of the problem being addressed, VGG-16 always benefits from the presence of BN, while ResNet-50 always benefits from its absence. Therefore, the recommendation is to test if BN is beneficial with a selected network and, if so, it is not necessary to carry out numerous experiments in multiple datasets, given that our experiments indicate that this behavior can generalize to other problems. In relation to dropout, its use is always either beneficial or not harmful, so its use is recommended, preferably in FC1 and FC2. Section 5.6, that includes the discussion of the results has been extended with these ideas and comments (see~\refcm{BNandDO}).  }

\qa{Fig. 4, it is a good practise to ensure that the bars in the plot can be distinguished when printed in black\&white. I would suggest using patterns to fill in the bars instead of plain colours.}
{We followed this suggestion. Fig.~\ref{medianImprovements} (formerly Fig.4) uses patterns instead of plain colors.}

\typo{Page 2, line 15: "... let alone..." should be "...letting alone..."}{ Corrected. }
 \end{answerreviewer}

\begin{answerreviewer}[Author Should Prepare A Major Revision For A Second Review]
\ca{The paper is very well-written. The motivation, in the introduction, is clear. The related work is fine. The method and results are also well-presented. The paper presents one of the first complete analysis on the problem. The examined datasets are relative small which allows several repetitions of the experiments. The presented statistical tests could define a baseline of analysis for future works.}
{We thank the reviewer for accurately summarizing the strengths of the submitted manuscript.}

\qa{The current standard on human-pose estimation and keypoint localization, in general, is heatmap regression. The authors skip to perform the analysis on this type of output representation.}
{We followed the reviewer's recommendation and added an analysis of the impact of using heatmaps as the target representation. We discuss this together with the previously used input representations in~\refcm{tir-desc}, and their impact on the performance, ~\refcm{results-tir}.}

\qa{It would increase support the paper to perform the same experiments on main-stream and current datasets such as MPII human pose or coco human-pose. }
{Experiments on the MPII dataset, briefly described in~\refcm{mpii-desc}, for all the network variants, including comparison with the state of the art, and including heatmap regression are now reported. See Figures~\ref{fig:optimizers}, ~\ref{fig:batch} and \ref{fig:dropout-rate}, as well as the last rows of Tables~\ref{tab:VGG-resnet-loss}, \ref{tab:VGG-resnet-BN}, \ref{tab:VGG-dropout},  \ref{tab:VGG-ResNet-FTDepth}, \ref{tab:VGG-RegFrom}, \ref{tab:resnet-RegFrom}, and \ref{tab:TIR}. The discussion accompanying each of the tables has been updated according to the new results (\refcm{mpii-anal} and \refcm{mpii-anal2}). The MPII dataset has also been integrated in the general discussion in \refcm{mpii-disc}. It is very important to notice that all these extensions of the experimental section have considerably increased the amount of experiments performed (see the updated figures in Section \ref{sec:comp_env}). The overall computation time needed to run all these experiments was of 46 days of GPU.}

\qa{The impact of dropout or batch-normalization is known to the community. The same holds for data augmentation. As a result, many of the paper results are interesting, but at the same time known to the community. This reduces the interest of the reader (when he/she is familiar with the topic). Weight normalization and layer normalization could be also considered for analysis, since they are recent advances and less explored.}
{We partially agree. Although it is true that some of the results are known, our submission appears to be the first comprehensive approach study of deep regression methods and their empirical validation on statistical grounds. In addition, many researchers, engineers and practitioners may not be aware of the paper's results. First, empirical evidence that data processing is much more decisive than other design choices (like fine-tuning or the regressed layer); second, the fact that a ``general purpose'' network (e.g. VGG-16 or ResNet-50) tuned in an adequate way can achieve results close to the state-of-the-art without having to resort to much more complex models. Apart from what was already included in Section \ref{sec:application},  these contributions are noe more clearly stated in the abstract of the paper. Following the reviewer's advice, we have introduced layer normalization as an alternative method to batch normalization in the final comparison. Results are reported in Table~\ref{tab:VGG-resnet-BN} and discussed in \refcm{BNLN} and in \refcm{BNandDO}. In relation to weight normalization, it is important to notice that it represents a novel training algorithm, and not a normalization strategy. Moreover, the use of weight normalization is complementary to the choice of an optimizer, and would require the evaluation of all four optimizers, now including weight normalization. We let this for future research and thank the reviewer for this suggestion.}
% 
% Therefore, it should be include in the section devoted to the comparison of optimizers. Since Section \ref{sec:optimization} already includes four different optimization algorithms, and since, when using weight normalization, we would still need to choose an optimizer, thus doubling the number of lines in Figures \ref{fig:optimizers} and \ref{fig:batch}, we consider this change would make the presentation of results confusing and too overwhelming. In conclusion, we did not include weight normalization in this paper, and we leave that comparison for further investigation. We thank the reviewer for this valuable suggestion. }

\qa{The presented analysis is important for building a deep model for regression. However, it cannot scale on large datasets (also mentioned by the authors). As a result, the presented statistical tests would not be easily adapted to ImageNet-scale datasets. This is a point of discussion, which is not addressed in the paper. How could one use the presented tests on large scale?}
{The only reason four which our methodology would be difficult to implement with massive datasets is the computation time needed by the experiments. In order to rigorously evaluate the results, we repeated several times each training, with the implications this has in terms of computation time. By obtaining different runs of the same experiment, we can evaluate the stability of the results and calculate confidence intervals. From this point of view, the only way to proceed would be to use a higher computing capacity (multi-GPU environments) or to decrease the degree of scientific rigor (not recommended when facing sound scientific studies). The reviewer explicitly mentions the difficulties of applying statistical tests with large datasets. We disagree with the reviewer, since the statistical test (in this case, the Wilcoxon signed-rank test) is independent of the size of the dataset. }%{\color{red}Should we include some of this discussion in the manuscript? I think we can seem a bit silly, because it's quite obvious that one can indistinctly apply Wilcoxon to two vectors of 100 or 10.000.000 elements...}

\qa{In overall, the current limitations of the paper are the lack of following the current regression trends (i.e. heatmaps instead of vectors) and evaluation on standard human pose or facial keypoint datasets.}
{We addressed these concerns, as discussed above, by adding experiments with the MPII dataset and by benchmarking the use of heatmap regression as an output representation. In particular, we employed architectures directly inspired by state of the art methods for full-body pose estimation \cite{Belagiannis2017recurrent,cao2016realtime} while keeping network architectures similar to baseline models in order to keep the comparison as fair as possible. From these additional experiments, we reached the interesting conclusion that heatmaps produce less good results than vanilla regression approaches and than the other input and target representations. On the FLD dataset the networks are able to converge and return reasonable predictions. Conversely, in the case of the Parse and MPII datasets, heatmap-based models do not perform well even on the training sets, indicating optimization issues. We tested with different learning rates and optimizers and obtained similar behaviors.
This shows that it is necessary to resort to more sophisticated and somehow ad-hoc strategies, e.g.\cite{Belagiannis2017recurrent,Nie_2018_CVPR,tompson2014joint,Chen2017AdversarialPA,Chu2017multi}, to obtain good performance with heatmap regression.
In addition, we investigated architectures based on an encoder-decoder architecture inspired by \cite{newell2016stacked} and observed a similar behavior. For the sake of conciseness, we chose to report results only using the encoder based architecture inspired from \cite{Belagiannis2017recurrent,cao2016realtime}. We discuss in detail results and possible explanations in ~\refcm{results-tir}. 
}
\end{answerreviewer}

\end{coverletter}

\twocolumn


==> cover_letter_r2.tex <==
\onecolumn

\begin{coverletter}{A Comprehensive Analysis of Deep Regression}{TPAMI-2018-03-0223}
 \begin{answereditor}{Please accompany the revised version with a detailed summary of how you addressed every comment by the reviewers (or explanation why any of the comments should not be addressed, e.g., if you disagree).}
We appreciate the comments and proposals made by the reviewers. We have thoroughly reviewed the document accordingly, which we hope that it substantially improved the initial submission. In general terms, the experimental section was considerably extended. First, a new dataset (MPII) was introduced in the comparison section. Second, other loss functions (L1, Huber) and normalization strategies (layer normalization) were included. Finally, other output representations were considered for the regression task (heat maps). In relation to the writing, we introduced clarifications and corrections throughout the document. We hope that all these modifications satisfy the reviewers. 

Below, we provide precise answers to the questions and issues raised by the reviewers, and we outlined in green all the modifications introduced in the manuscript.
 \end{answereditor}

\begin{answerreviewer}[Author Should Prepare A Minor Revision]
\qa{The authors have done a great effort to answer to the questions previously posed by the reviewers in a satisfactory manner. However, to keep uniform all the experiments presented in the paper, I miss the results obtained for MPII dataset in Tables 9 and 10. As MPII is larger than Parse dataset, the results obtained on it would greatly benefit the research community. So, I would kindly ask to include them before finally accepting this interesting paper.}
{Tables 9 and 10 now include results using MPII together with their statistical significance. The description of the experiment and the discussion of the results obtained have been included in page 11 and 12. Finally, Figure 5.d now includes the data pre-processing in the histogram. Similarly to the three other datasets, we observe that data pre-processing is crucial for the performance.}

\qa{Typo:
 - Page 7, Sec. 5.1: "Table 2 preesents..." $\rightarrow$ presents}
{This typo has been fixed.}

\end{answerreviewer}

\begin{answerreviewer}[Accept With No Changes]
\ca{ The authors have integrated the recommended changes from the reviews. The additional experiments on heatmaps and MPII dataset are now part of the evaluation. This adds an important value to the paper. The new evaluations provide interesting insights regarding the widely-used heatmap representation and standard regressors. The work now is complete and  could accepted as is.}
{We thank the reviewer for acknowledging our work for improving the paper.}
\end{answerreviewer}

\end{coverletter}

\twocolumn


==> notes.tex <==
8 runs on biwi with adagrad whithout BN (run ids=147095..147102)
\begin{verbatim}
('Mean absolute error:', array([ 7.98190715,  5.16760045,  6.18648489]), 6.4453308322482838)
('Mean absolute error:', array([ 7.56045271,  5.6208003 ,  6.18951464]), 6.4569225484082153)
('Mean absolute error:', array([ 6.11432228,  6.6057522 ,  5.74507869]), 6.1550510601368034)
('Mean absolute error:', array([ 7.49758318,  5.31258587,  5.64761478]), 6.1525946097303539)
('Mean absolute error:', array([ 6.2723985 ,  5.70768193,  5.60976405]), 5.8632814942237728)
('Mean absolute error:', array([ 7.70719525,  4.7412574 ,  5.85488254]), 6.101111729265682)
('Mean absolute error:', array([ 9.03354215,  5.41179903,  6.38856949]), 6.9446368915256604)
('Mean absolute error:', array([ 7.07780933,  5.98737397,  6.30257731]), 6.4559202031373388)

\end{verbatim}
\begin{verbatim}
/perception/slathuil/log/scriptCluster_$i.output; done
Regression experiments
-bn -ft 0
148066
('Mean square error:', array([ 81.20383105,  37.04689578,  56.0598156 ]), 58.103514144500899)
('Mean absolute error:', array([ 7.40112895,  4.77480724,  5.27060455]), 5.8155135806145681)
('Explained variances score:', array([ 0.90643816,  0.96910763,  0.65602173]))
Regression experiments
-bn -ft 0
148067
('Mean square error:', array([ 95.68213402,  37.76579384,  55.89422786]), 63.114051906550742)
('Mean absolute error:', array([ 8.21695884,  4.79275672,  5.38065378]), 6.1301231154378071)
('Explained variances score:', array([ 0.89124599,  0.96856522,  0.65600469]))
Regression experiments
-bn -ft 0
148068
('Mean square error:', array([ 89.70759793,  39.07289801,  52.98142658]), 60.587307506463198)
('Mean absolute error:', array([ 7.6600563 ,  4.87779762,  5.28271632]), 5.9401900814799804)
('Explained variances score:', array([ 0.88477764,  0.96739339,  0.67268395]))
Regression experiments
-bn -ft 1
148069
('Mean square error:', array([ 44.26593258,  40.72852753,  22.57777778]), 35.857412627875483)
('Mean absolute error:', array([ 5.4896811 ,  4.73790366,  3.2292944 ]), 4.4856263886785008)
('Explained variances score:', array([ 0.96631182,  0.96648613,  0.86062531]))
Regression experiments
-bn -ft 1
148070
('Mean square error:', array([ 40.63157782,  60.50311017,  27.99741581]), 43.044034596096623)
('Mean absolute error:', array([ 5.26786798,  6.04173339,  3.66729138]), 4.9922975835012897)
('Explained variances score:', array([ 0.97244878,  0.94956153,  0.83195322]))
Regression experiments
-bn -ft 1
148071
('Mean square error:', array([ 28.01794133,  78.35344663,  48.58642833]), 51.65260543136111)
('Mean absolute error:', array([ 3.70710261,  6.21962195,  5.07571146]), 5.0008120071949724)
('Explained variances score:', array([ 0.96648756,  0.93468358,  0.69932534]))
Regression experiments
-bn -ft 2
148072
('Mean square error:', array([ 73.61658641,  47.9246521 ,  33.70471829]), 51.748652264558338)
('Mean absolute error:', array([ 7.40789054,  5.05715793,  4.51173331]), 5.6589272624305709)
('Explained variances score:', array([ 0.94951073,  0.96269324,  0.79165386]))
Regression experiments
-bn -ft 2
148073
('Mean square error:', array([ 58.62847538,  52.15005444,  31.62360396]), 47.46737792869083)
('Mean absolute error:', array([ 6.05216966,  5.78475138,  4.44161838]), 5.4261798045483021)
('Explained variances score:', array([ 0.94316916,  0.95689967,  0.80647643]))
Regression experiments
-bn -ft 2
148074
('Mean square error:', array([ 107.87087226,  123.50001739,   41.18976471]), 90.85355145408046)
('Mean absolute error:', array([ 8.79924308,  8.29494346,  4.73408373]), 7.2760900921706231)
('Explained variances score:', array([ 0.94015488,  0.89705079,  0.7481515 ]))
Regression experiments
-bn -rf conv
148075
('Mean square error:', array([ 44.48821931,  36.15141108,  38.65429726]), 39.764642551742263)
('Mean absolute error:', array([ 5.30748406,  4.45938176,  4.91447382]), 4.8937798798235503)
('Explained variances score:', array([ 0.95801702,  0.96996628,  0.77989266]))
Regression experiments
-bn -rf conv
148076
('Mean square error:', array([ 125.80502006,   76.56984665,   60.5044536 ]), 87.626440105630294)
('Mean absolute error:', array([ 8.96857044,  6.10493258,  6.06834597]), 7.0472829975323625)
('Explained variances score:', array([ 0.91450987,  0.93634683,  0.6385366 ]))
Regression experiments
-bn -rf conv
148077
('Mean square error:', array([ 55.612975  ,  50.78115081,  56.68033745]), 54.358154421634147)
('Mean absolute error:', array([ 6.04298555,  5.66837638,  6.09715806]), 5.9361733253152345)
('Explained variances score:', array([ 0.95893624,  0.9576184 ,  0.658406  ]))
Regression experiments
-bn -rf fc1
148078
('Mean square error:', array([ 2231747.48520004,    90558.96113412,   693946.96113105]), 1005417.8024884025)
('Mean absolute error:', array([ 102.43149226,   24.86644517,   58.38517017]), 61.894369200555637)
('Explained variances score:', array([-3070.00777117,   -74.2541101 , -4275.930697  ]))
Regression experiments
-bn -rf fc1
148079
('Mean square error:', array([ 88704.10979525,  20007.01690403,  18696.26460933]), 42469.130436202235)
('Mean absolute error:', array([ 25.29307941,  14.90659229,  13.8860307 ]), 18.028567467509426)
('Explained variances score:', array([-120.79740303,  -15.58268467, -113.89080464]))
Regression experiments
-bn -rf fc1
148080
('Mean square error:', array([ 228301.90629242,   19078.50646183,    5345.38864982]), 84241.933801357169)
('Mean absolute error:', array([ 25.96030618,  12.98729151,   7.85235381]), 15.599983830819545)
('Explained variances score:', array([-314.32110129,  -14.91161269,  -31.98507706]))
Regression experiments
-bn -bs 16
148081
('Mean square error:', array([ 31.38808388,  41.98107674,  31.88362729]), 35.084262636918162)
('Mean absolute error:', array([ 4.13329486,  4.63242312,  4.13579687]), 4.3005049493144067)
('Explained variances score:', array([ 0.96439531,  0.96514745,  0.80324475]))
Regression experiments
-bn -bs 16
148082
('Mean square error:', array([ 49.71687218,  34.4213418 ,  29.97992747]), 38.039380481963228)
('Mean absolute error:', array([ 5.49262137,  4.46405486,  3.89406389]), 4.6169133744072406)
('Explained variances score:', array([ 0.95765014,  0.97131671,  0.81576561]))
Regression experiments
-bn -bs 16
148083
('Mean square error:', array([ 38.12110419,  29.47736204,  29.77071352]), 32.456393251541805)
('Mean absolute error:', array([ 4.6847201 ,  4.08772276,  3.72143713]), 4.1646266633295221)
('Explained variances score:', array([ 0.95665183,  0.97539994,  0.81617976]))
Regression experiments
-bn -bs 32
148084
('Mean square error:', array([ 35.25098805,  76.25035593,  21.13900732]), 44.213450432412372)
('Mean absolute error:', array([ 4.28466367,  7.09047034,  3.32780833]), 4.9009807777341683)
('Explained variances score:', array([ 0.96142716,  0.93763119,  0.87202536]))
Regression experiments
-bn -bs 32
148085
('Mean square error:', array([ 35.1356644 ,  41.71995514,  35.83354305]), 37.563054195892924)
('Mean absolute error:', array([ 4.44727413,  4.84822447,  4.40997787]), 4.5684921587232017)
('Explained variances score:', array([ 0.95647255,  0.96549406,  0.78305985]))
Regression experiments
-bn -bs 32
148086
('Mean square error:', array([ 33.58169964,  42.80934314,  21.58630614]), 32.659116306114399)
('Mean absolute error:', array([ 4.45508031,  4.89608632,  3.3557564 ]), 4.2356410116387879)
('Explained variances score:', array([ 0.96958265,  0.96524482,  0.87014284]))
Regression experiments
-bn -bs 64
148087
('Mean square error:', array([ 47.31704247,  58.64304197,  23.44756051]), 43.135881649598673)
('Mean absolute error:', array([ 5.23658565,  5.88124789,  3.61286135]), 4.9102316288446755)
('Explained variances score:', array([ 0.96617148,  0.95118517,  0.86133696]))
Regression experiments
-bn -bs 64
148088
('Mean square error:', array([ 35.35226971,  60.12188322,  25.68935953]), 40.387837484870545)
('Mean absolute error:', array([ 4.67169885,  5.89439647,  3.60875297]), 4.7249494308585263)
('Explained variances score:', array([ 0.97008855,  0.95031019,  0.84130955]))
Regression experiments
-bn -bs 64
148089
('Mean square error:', array([ 37.0157646 ,  50.21643713,  24.55912032]), 37.263774017203708)
('Mean absolute error:', array([ 4.70870429,  5.44763451,  3.56865187]), 4.5749968901748268)
('Explained variances score:', array([ 0.96476047,  0.96199263,  0.84815849]))
\end{verbatim}
\begin{verbatim}
Regression experiments
-bn -ft 0
148138
        3.69876853,  3.57556601,  3.51306473,  3.60800017,  3.58385784]), 3.3759841407605884)
('Explained variances score:', array([ 0.832518  ,  0.72226392,  0.8266085 ,  0.71889693,  0.91430592,
        0.63173138,  0.81518818,  0.73686099,  0.81177413,  0.72528921]))
Regression experiments
-bn -ft 0
148139
        3.78189788,  3.77399754,  3.63015188,  3.69035397,  3.66552992]), 3.461884581900081)
('Explained variances score:', array([ 0.82339664,  0.72515288,  0.81354237,  0.71841374,  0.91020262,
        0.6166186 ,  0.80923232,  0.71753779,  0.80326101,  0.70973428]))
Regression experiments
-bn -ft 0
148140
        3.83902664,  3.58755292,  3.57007197,  3.60107772,  3.60861148]), 3.4034170195685673)
('Explained variances score:', array([ 0.82910587,  0.72595889,  0.82579419,  0.72094066,  0.91296015,
        0.61902669,  0.81267805,  0.73029234,  0.81578225,  0.71861543]))
Regression experiments
-bn -ft 1
148141
        2.16118183,  2.35670985,  2.19695673,  2.33183319,  2.15812534]), 2.108461956430546)
('Explained variances score:', array([ 0.9193282 ,  0.90014808,  0.92112545,  0.90305512,  0.96644343,
        0.87034054,  0.92004489,  0.89405472,  0.9194459 ,  0.89893775]))
Regression experiments
-bn -ft 1
148142
        2.47936483,  2.50730216,  2.59818163,  2.79552191,  2.45536111]), 2.4465800649639129)
('Explained variances score:', array([ 0.90857299,  0.86571106,  0.86479907,  0.86976331,  0.95760286,
        0.83182249,  0.90687065,  0.85501245,  0.89064822,  0.86166317]))
Regression experiments
-bn -ft 1
148143
        2.043773  ,  2.33582665,  2.3069725 ,  2.52402895,  2.20763908]), 2.1620404342140014)
('Explained variances score:', array([ 0.9336187 ,  0.89497606,  0.91959431,  0.86392179,  0.96358094,
        0.88630009,  0.91961574,  0.88843305,  0.91573261,  0.89223984]))
Regression experiments
-bn -ft 2
148144
        1.71349483,  1.98344095,  1.90577005,  1.94810754,  1.74648982]), 1.625560531670039)
('Explained variances score:', array([ 0.96026988,  0.94582386,  0.95672669,  0.94104963,  0.98124633,
        0.93507387,  0.941768  ,  0.93120844,  0.94454863,  0.93440873]))
Regression experiments
-bn -ft 2
148145
        1.90730069,  2.30643394,  2.27757826,  2.19821535,  2.07884363]), 1.9484033590784797)
('Explained variances score:', array([ 0.94784562,  0.9019309 ,  0.93388698,  0.92686298,  0.97286841,
        0.90637422,  0.93486848,  0.89728495,  0.92512979,  0.90645367]))
Regression experiments
-bn -ft 2
148146
        1.66993147,  2.05633324,  1.96682843,  2.06831053,  1.88413719]), 1.7831503024658659)
('Explained variances score:', array([ 0.95444477,  0.93549658,  0.9395625 ,  0.93693063,  0.9746014 ,
        0.91517059,  0.93811545,  0.91306017,  0.93285073,  0.9201791 ]))
Regression experiments
-bn -rf conv
148147
        2.31264948,  2.28179891,  2.00752695,  2.52437921,  2.01894295]), 2.0660990152485761)
('Explained variances score:', array([ 0.93828267,  0.89875743,  0.92954984,  0.91413279,  0.96269046,
        0.89720114,  0.9282044 ,  0.90746515,  0.92505307,  0.907138  ]))
Regression experiments
-bn -rf conv
148148
        2.38273849,  2.53473283,  2.67480633,  2.52309156,  2.81377299]), 2.3123006227191869)
('Explained variances score:', array([ 0.82829797,  0.49253516,  0.46388031,  0.62973406,  0.90697489,
        0.32400613,  0.68778925,  0.22707028,  0.61854895,  0.3079775 ]))
Regression experiments
-bn -rf conv
148149
        1.86644431,  2.19903208,  2.03958139,  2.35222469,  1.99167748]), 1.9603670744966446)
('Explained variances score:', array([ 0.93328004,  0.91531527,  0.93358984,  0.92257781,  0.96830898,
        0.90108271,  0.92601491,  0.9109689 ,  0.92144316,  0.9096587 ]))
Regression experiments
-bn -rf fc1
148150
        2.06038154,  2.1782036 ,  2.53775439,  2.81482063,  2.59918959]), 2.2036266569627729)
('Explained variances score:', array([ 0.92803125,  0.91237154,  0.91282543,  0.90658261,  0.96394581,
        0.87406425,  0.93189833,  0.88908294,  0.91190732,  0.89407553]))
Regression experiments
-bn -rf fc1
148151
        1.88347264,  2.16728062,  2.18365058,  2.27288493,  2.13655106]), 1.9579775884525965)
('Explained variances score:', array([ 0.92041381,  0.87323147,  0.87631462,  0.87679196,  0.95036524,
        0.83030733,  0.90670437,  0.82123408,  0.85792141,  0.78480435]))
Regression experiments
-bn -rf fc1
148152
        2.29153103,  2.58887425,  2.61494048,  3.20195587,  2.62005006]), 2.5828189693179149)
('Explained variances score:', array([ 0.11702258, -1.82848513, -5.26664075, -1.53417484,  0.23399505,
       -2.42195156, -0.42174336, -4.16629956, -3.35690808, -4.50911894]))
Regression experiments
-bn -bs 16
148153
        2.04832644,  2.33223861,  2.02825425,  2.24071727,  2.06945886]), 1.988345347686489)
('Explained variances score:', array([ 0.93825201,  0.9102846 ,  0.92872286,  0.91732834,  0.96899461,
        0.89338417,  0.93022898,  0.91217579,  0.93096441,  0.91010684]))
Regression experiments
-bn -bs 16
148154
        1.94710995,  2.15663823,  2.0627545 ,  2.3946629 ,  1.93175654]), 1.9854531000694018)
('Explained variances score:', array([ 0.9344347 ,  0.90541399,  0.9299283 ,  0.91216821,  0.96773333,
        0.88921144,  0.92974903,  0.90755202,  0.92237631,  0.91743604]))
Regression experiments
-bn -bs 16
148155
        1.8547458 ,  2.10766679,  1.81264662,  2.25713931,  1.89925227]), 1.9063192548870149)
('Explained variances score:', array([ 0.94172208,  0.92835876,  0.93607887,  0.91356932,  0.96662493,
        0.90494093,  0.93235758,  0.92618542,  0.92545762,  0.92014399]))
Regression experiments
-bn -bs 32
148156
        1.94867199,  2.33500952,  1.93163497,  2.33711618,  1.95114611]), 1.992180273547342)
('Explained variances score:', array([ 0.93319349,  0.90151077,  0.92604962,  0.90583886,  0.96456982,
        0.88781761,  0.92313126,  0.9161036 ,  0.91977217,  0.91333843]))
Regression experiments
-bn -bs 32
148157
        4.92533866,  3.7710793 ,  4.74875814,  5.08021606,  4.97004626]), 4.2369372310668121)
('Explained variances score:', array([ 0.84794744,  0.67328629,  0.6528994 ,  0.63530304,  0.9156604 ,
        0.39650475,  0.79704611,  0.52867276,  0.70310254,  0.46048737]))
Regression experiments
-bn -bs 32
148158
        2.11112581,  2.29838087,  2.4120071 ,  2.42452153,  2.21185967]), 2.1440630358957655)
('Explained variances score:', array([ 0.93440727,  0.89800621,  0.9246962 ,  0.90217237,  0.96559571,
        0.88701247,  0.92360874,  0.89575952,  0.9212789 ,  0.90048298]))
Regression experiments
-bn -bs 64
148159
        1.75189694,  2.46757175,  1.84487981,  2.20286161,  1.82934983]), 1.8647248170031001)
('Explained variances score:', array([ 0.95118646,  0.91802539,  0.94538129,  0.92649895,  0.97196537,
        0.91293212,  0.93538173,  0.92106071,  0.92777449,  0.923871  ]))
Regression experiments
-bn -bs 64
148160
        1.88770648,  2.21471565,  1.94395284,  2.18964293,  1.96211299]), 1.9385271264231867)
('Explained variances score:', array([ 0.94323101,  0.9180952 ,  0.9397903 ,  0.91861748,  0.9645248 ,
        0.90140515,  0.92598024,  0.91396419,  0.92851087,  0.91352402]))
Regression experiments
-bn -bs 64
148161
        2.07187646,  2.3409526 ,  2.00245181,  2.34080858,  2.01877387]), 2.0331960373991018)
('Explained variances score:', array([ 0.93379552,  0.90449729,  0.92692377,  0.90502282,  0.96719339,
        0.87902426,  0.92033552,  0.90959327,  0.92229703,  0.90785327]))
\end{verbatim}



\begin{table}[h]
\centering
 \caption{Optimizer on biwi without BN(147195..147202 and 147423..147430)(147866..147879)\label{tab:results-fld}}
 \begin{tabular}{lcc|ccc|c}
   & MAE training&MAE test&MSE training& MSE validation &MSE test& Epochs \\

   SGD\_1e-2&&nan/nan  & & &  &  \\
   SGD\_1e-3&& nan/nan & & &   &\\
   SGD\_1e-4&&nan/nan  & & &   & \\

   Adagrad& &7.52/9.32/9.83/14.43 &21.80/114.87 &  59.39/107.02& 98.54/143.74  &39/6  \\
   Adadelta& & 6.29/6.46/6.41/7.39& 4.26/6.03&49.33/45.32 &67.14/74.23 &18/10   \\
   Adam& & 19.14/19.15/7.91/19.15& 584.96/585.1.5&472.36/477.85 &694.87/695.12&5/9    \\
   RMSProp& & 6.54/6.55/19.16/6.18& 8.91/12.57& 41.72/55.46&78.89/74.51 &16/12   \\
 \end{tabular}
\end{table}

\begin{table}[h]
\centering
 \caption{Optimizer on biwi with BN()(147880..14793)\label{tab:results-fld}}
 \begin{tabular}{lcc|ccc|c}
    & MAE training&MAE test&MSE training& MSE validation &MSE test& Epochs \\

   SGD\_1e-2& &nan/nan & & &  &  \\
   SGD\_1e-3& &15.49/8.53 &390.28/81.58 &286.60/120.26 &433.57/120.26  &1/10  \\
   SGD\_1e-4& &4.02/4.19 &9.38/7.46 &28.17/26.89 &27.47/28.69  &20/24  \\
   Adagrad& &5.63/5.13/5.80/5.12&9.57/10.52 &24.29/26.38 &52.64/45.08  &11/8  \\
   Adadelta& & 5.56/5.49/5.16/7.44&13.63/11.53 &22.42/24.85 &55.32/49.32  & 5/8  \\
   Adam& & 4.37/4.07/5.33/4.93& 8.99/10.52&20.73/25.27 & 35.71/30.50 &24/18  \\
   RMSProp& & 3.86/4.57/5.41/8.17& 11.27/10.22& 26.12/25.27& 28.00/36.85 &11/14  \\
 \end{tabular}
\end{table}




\begin{table}[h]
\centering
 \caption{Optimizer on Facial without BN(148038..148051 )\label{tab:results-fld}}
 \begin{tabular}{lcc|cc|cc}
   & MAE training&MAE test&MSE training& MSE validation &MSE test& Epochs \\

   SGD\_1e-2& &nan/nan & & &  &  \\
   SGD\_1e-3& &nan/nan & & &  &  \\
   SGD\_1e-4& &nan/nan & & &  &  \\

   Adagrad& &6.55/5.93 &65.90/98.98 &68.64/59.68 &71.74/58.79  &28/16  \\
   Adadelta& & 18.71/5.62& 1.64e+6/114.91 &552.66/44.48 &542.84/44.36  &1/15  \\
   Adam& &7.65/7.65 &117.09/116.89 & 107.29/106.92&106.73/106.77  & 2/2 \\
   RMSProp& & 8.10/17.95&1286.21/21509.87 &116.48/526.50 &116.26/512  &3/5  \\
 \end{tabular}
\end{table}

\begin{table}[h]
\centering
 \caption{Optimizer on Facial with BN(148052..148065 )\label{tab:results-fld}}
 \begin{tabular}{lcc|cc|cc}
      & MAE training&MAE test&MSE training& MSE validation &MSE test& Epochs \\

   SGD\_1e-2& &7.01/7.67 &38.12/110.10 &85.45/109.26 &95.51/107.5  &5/4  \\
   SGD\_1e-3& &2.38/3.88 &11.51/28.41 &10.16/27.44 & 10.28/27.03  & 11/13 \\
   SGD\_1e-4& &1.91/1.85 &7.21/6.44 & 6.35/5.98& 6.65/6.23 & 38/44 \\
   Adagrad& &1.90/2.01&6.26/7.93 &6.33/7.36 &6.77/6.07  &38/22  \\
   Adadelta& &2.32/1.93& 12.71/9.31&9.47/6.51 &9.65/6.95  &8/19  \\
   Adam& & 1.83/2.13&6.38/10.47 &5.84/7.90 & 6.37/8.34 &40/16  \\
   RMSProp& & 2.06/6.16& 7.40/49.61 & 7.34/67.32 &7.71/67.04  & 31/4 \\
 \end{tabular}
\end{table}


\begin{table}[h]
\centering
 \caption{Best caption ever\label{tab:BN}}
 \begin{tabular}{l|c|cc|cc|cc}
   Dataset & Batch Normalizer& MAE training&MAE test&MSE training& MSE test& Specific training&
   Specific test \\
   Landmark&yes& & & & &  &  \\
   Landmark&no& & & & &  &  \\
   LSP&yes& & & & &  &  \\
   LSP&no& & & & &  &  \\
   FGNet&yes& & & & &  &  \\
   FGNet&no& & & & &  &  \\
 \end{tabular}
\end{table}

\begin{figure*}[t]
  \centering
  \subfloat[Biwi]{\hspace{-2mm}
    \includegraphics[width=0.33\textwidth]{figures/lossBiwi.pdf}
    \label{lBiwi}
  }
  \subfloat[Landmarks]{
  \includegraphics[width=0.33\textwidth]{figures/lossLandmarks.pdf}
    \label{lLand}
  }
  \subfloat[Parse]{
  \includegraphics[width=0.33\textwidth]{figures/lossParse.pdf}
    \label{lParse}
  }\vspace{-3mm}
  \caption{Failure rate on fashion landmark detection on the different subsets of FLD as a function of the distance 
threshold.}
\label{fig:fashion-curves}
\end{figure*}


==> related.tex <==
\section{Related Works}
Seminal papers exploring efficient backpropagation strategies \cite{LeCunBOM98} and evaluating  ConvNets  for  visual recognition \cite{Nebauer1998} were already published 20 years ago.  However, recent research in the deep learning field has produced an overabundance of papers presenting either new deep models or existent deep models applied to new problems. Among all these papers, some of them try to provide general guidance and understanding on appropriate architectural choices \cite{SzegedyVISW16,SmithT16,IthapuRS17} or on gradient-based training strategies for deep architectures \cite{bengio2012}, while others try to delve into the differences in performance of the variants of a specific model \cite{GreffSKSS17} or the differences in performance of several models applied to a specific problem \cite{ChandrasekharLM16}. There are also some papers presenting models that try to select the optimal ConvNet architecture in an automatic fashion \cite{SaxenaV16,XieY17}, but those works do not usually focus on discovering the underlying empirical or theoretical principles for designing neural network architectures. 

Among all prior art, the closest work to ours possibly is \cite{MISHKIN2017}, where the authors systematically study the impact of several advances in ConvNets, including non-linearity, pooling variants, network width, classifier design, image pre-processing, and learning parameters. However, the aforementioned paper is devoted to the object categorization problem and does not tackle regression problems at all. Furthermore, there is an absence in the literature of using confidence intervals and statistical tests to measure the uncertainty of the results obtained. 

%Still need to be cited:
%\begin{itemize}
%\item Chapter 11 of the Deep Learning book
%\item Convolutional Neural Fabrics
%\item Learning to learn by gradient descent by gradient descent
%\item Deep Speech 2: End-to-End Speech Recognition in English and Mandarin. Comparison for the speech recognition task. Many experiments to tune the architecture for this task.
%\end{itemize}

==> resultProtocoldata.tex <==

\subsection{Result: Data augmentation}


\begin{table}[h!]
\centering
 \caption{Impact of data processing on VGG16 }
 \begin{tabular}{l|l|ccc|}
   &MAE test&MSE training& MSE validation &MSE test \\
   \hline
   {\color{green}Biwi: baseline}  & [3.42 3.49]*** & [3.00 3.07] & [11.51 11.98] & [15.87 16.63] \\ 
   Biwi: 128 mean padding & [6.16 6.33] & [14.95 15.34] & [25.99 27.30] & [52.27 55.37] \\ 
Biwi: 128 resize & [4.91 5.05] & [8.40 8.63] & [15.68 16.57] & [33.48 35.60] \\ 
Biwi: 128 zero padding & [4.69 4.80] & [9.87 10.15] & [18.58 19.52] & [30.04 31.26] \\ 
Biwi: 64 mean padding & [4.90 5.03] & [14.44 14.76] & [27.66 28.99] & [32.07 33.82] \\ 
Biwi: 64 resize & [4.42 4.53] & [9.07 9.31] & [18.15 19.00] & [27.13 28.58] \\ 
Biwi: 64 zero padding & [5.61 5.79] & [18.20 18.73] & [30.08 31.48] & [43.56 46.26] \\ 

   \hline
   FLD: max  &   \\ 
   FLD: avg  & \\ 
   {\color{green}FLD: FC2} &  \\ 
   
   \hline
   Parse: max  &  \\ 
    Parse: avg  &  \\ 
    {\color{green}Parse: FC2} &  \\ 

    \end{tabular}
    \label{tab:VGG-dataprocessing}
\end{table}


\begin{table}[h!]
\centering
 \caption{Impact of data processing on ResNet50 }
 \begin{tabular}{l|l|ccc|}
   &MAE test&MSE training& MSE validation &MSE test \\
   \hline
   {\color{green}Biwi: baseline}  &  [3.99 4.09] & [1.06 1.08] & [22.72 23.71] & [20.94 22.08] \\  
Biwi: 128 mean padding & [3.81 3.93] & [1.03 1.05] & [19.67 20.54] & [19.90 20.93] \\ 
Biwi: 128 resize & [3.38 3.49] & [1.07 1.09] & [14.82 15.58] & [15.17 16.04] \\ 
Biwi: 128 zero padding & [3.27 3.34] & [1.63 1.66] & [18.04 18.82] & [14.92 15.61] \\ 
Biwi: 64 mean padding & [3.66 3.77] & [1.45 1.48] & [20.88 21.73] & [18.45 19.73] \\ 
Biwi: 64 resize & [3.11 3.21]*** & [0.99 1.01] & [13.80 14.50] & [13.33 14.13] \\ 
Biwi: 64 zero padding & [3.73 3.83] & [3.37 3.44] & [19.57 20.48] & [19.09 20.22] \\ 

   \hline
   FLD: max  &   \\ 
   FLD: avg  & \\ 
   {\color{green}FLD: FC2} &  \\ 
   
   \hline
   Parse: max  &  \\ 
    Parse: avg  &  \\ 
    {\color{green}Parse: FC2} &  \\ 

    \end{tabular}
    \label{tab:ResNet-dataprocessing}
\end{table}

